Enhancing Single-Frame Supervision for Better Temporal Action Localization

Temporal action localization aims to identify the boundaries and categories of actions in videos, such as scoring a goal in a football match. Single-frame supervision has emerged as a labor-efficient way to train action localizers as it requires only one annotated frame per action. However, it often suffers from poor performance due to the lack of precise boundary annotations. To address this issue, we propose a visual analysis method that aligns similar actions and then propagates a few user-provided annotations (e.g. , boundaries, category labels) to similar actions via the generated alignments. Our method models the alignment between actions as a heaviest path problem and the annotation propagation as a quadratic optimization problem. As the automatically generated alignments may not accurately match the associated actions and could produce inaccurate localization results, we develop a storyline visualization to explain the localization results of actions and their alignments. This visualization facilitates users in correcting wrong localization results and misalignments. The corrections are then used to improve the localization results of other actions. The effectiveness of our method in improving localization performance is demonstrated through quantitative evaluation and a case study.

==> discussion.tex <==
\section{Expert Feedback}
% \label{sec:feedback}
% After case studies, we conducted an \red{interview} with experts to gather feedback.
% Overall, the feedback is positive.
% % They approximate the way to display edges, which help them 
% % \red{Advantage}
% $E_1$ pointed out that the way to add labels is impressive.
% Without visualization, they usually select uncertain samples to label.
% However, they found the accuracy gain is relatively small.
% \jw{With the visualization of edges, they found these uncertain samples often had wrong edges.}%as uncertain samples have wrong edges.
% Labeling such samples will lead to misclassification of other samples.
% Combining Label Change view with Sample view, he could find areas that really in need of labels, which brought a larger gain.
% $E_2$ said that filtering edges by importance can help him find the key wrong edges and understand the predictions made by the model.
% %Adding labels to samples with wrong edges may lead to misclassification of other samples.
% ``Deleting these wrong edges is the key to correct the wrong prediction here. Moreover, it comes with less cost than labeling.'' He said.
% % Edge importance also provide a new view of edges.
% % They know two samples will affect each other as edges in both direction exists.
% % However, with the edge importance, they know edges between two samples are not equally important.
% % ``For example, the edge pointing from a labeled sample to an unlabeled sample is obvious important than the edge in the other direction. It is easy to understand, but I do not notice it before. '' He said.
% % He think this may inspire future research to better understand SSL model.


% Although all experts appreciated the effectiveness of DataLinker, they also gave several suggestions for improvement.
% First, in many applications, there are too many unlabeled data, which bring pressure to the storage system.
% ``It would be helpful if the system can help reduce redundant data while still maintain the model performance'' mentioned $E_1$.
% % In real applications, data come in streaming form. It would be helpful to adjust the system to handling streaming data.
% Moreover, unlabeled data may come in over time.
% It would be helpful DataLinker can handle streaming data.
